The Influence of Down-Sampling Strategies on SVD Word Embedding Stability

The stability of word embedding algorithms, i.e., the consistency of the word representations they reveal when trained repeatedly on the same data set, has recently raised concerns. We here compare word embedding algorithms on three corpora of different sizes, and evaluate both their stability and accuracy. We find strong evidence that down-sampling strategies (used as part of their training procedures) are particularly influential for the stability of SVDPPMI-type embeddings. This finding seems to explain diverging reports on their stability and lead us to a simple modification which provides superior stability as well as accuracy on par with skip-gram embeddings.

==> results-table-all.tex <==
\begin{table*}[h]
%\scriptsize 
\footnotesize 
\centering
%\hspace*{-20pt}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Corpus} & \multirow{2}{*}{Algorithm} &   \multicolumn{2}{c|}{Down-sampling}  &  \multicolumn{4}{c|}{Word Similarity} & \multicolumn{2}{c|}{Analogy}  & \multirow{2}{*}{Stability} \\ 
 &  & distance & frequency & MEN & MTurk & SimLex & WS-353 & Google & MSR &  \\ \hline
 
 \multirow{12}{*}{COHA} & \multirow{9}{*}{\svdpmi} & \multirow{3}{*}{none} & prob. & 0.681 & 0.567 & 0.322 & 0.581 & 0.237 & 0.253 & 0.440\\
  &   &   & none & 0.697 & \textbf{0.582} & 0.318 & 0.591 & 0.248 & 0.226 & \textbf{1.000}\\
  &   &   & weight & 0.698 & 0.553 & 0.341 & \textbf{0.596} & 0.268 & 0.267 & \textbf{1.000}\\
  &   & \multirow{3}{*}{prob.} & prob. & 0.689 & \textbf{0.571} & 0.333 & 0.577 & 0.224 & 0.257 & 0.324\\
  &   &   & none & \textbf{0.703} & 0.571 & 0.328 & 0.591 & 0.246 & 0.243 & 0.441\\
  &   &   & weight & \textbf{0.703} & 0.568 & 0.349 & \textbf{0.593} & 0.259 & 0.277 & 0.475\\
  &   & \multirow{3}{*}{weight} & prob. & 0.688 & 0.567 & 0.331 & 0.582 & 0.232 & 0.260 & 0.424\\
  &   &   & none & 0.702 & 0.560 & 0.328 & 0.589 & 0.247 & 0.243 & \textbf{1.000}\\
  &   &   & weight & 0.702 & 0.551 & 0.351 & 0.594 & 0.262 & 0.277 & \textbf{1.000}\\
  & \multirow{2}{*}{\sgns} & \multirow{2}{*}{prob.} & prob. & 0.642 & 0.560 & 0.394 & 0.551 & 0.248 & 0.311 & 0.288\\
  &   &   & none & 0.660 & \textbf{0.578} & 0.347 & 0.561 & 0.259 & 0.301 & 0.282\\
  & \glove &   & weight & 0.590 & 0.522 & 0.222 & 0.405 & 0.167 & 0.214 & 0.808\\
  
  \hline 
\multirow{12}{*}{{\parbox{1cm}{\center COHA Subs.}}} & \multirow{9}{*}{\svdpmi} & \multirow{3}{*}{none} & prob. & 0.629 & 0.527 & 0.271 & 0.551 & 0.187 & 0.214 & 0.291\\
  &   &   & none & 0.645 & \textbf{0.537} & 0.267 & \textbf{0.569} & 0.192 & 0.184 & 0.310\\
  &   &   & weight & 0.645 & \textbf{0.546} & 0.295 & \textbf{0.564} & \textbf{0.212} & 0.228 & 0.325\\
  &   & \multirow{3}{*}{prob.} & prob. & 0.632 & 0.519 & 0.287 & 0.542 & 0.169 & 0.203 & 0.198\\
  &   &   & none & \textbf{0.648} & \textbf{0.529} & 0.280 & \textbf{0.559} & 0.185 & 0.188 & 0.217\\
  &   &   & weight & \textbf{0.652} & \textbf{0.529} & 0.307 & \textbf{0.564} & 0.204 & 0.228 & 0.251\\
  &   & \multirow{3}{*}{weight} & prob. & 0.635 & \textbf{0.533} & 0.284 & \textbf{0.549} & 0.180 & 0.212 & 0.274\\
  &   &   & none & \textbf{0.649} & \textbf{0.536} & 0.282 & \textbf{0.559} & 0.190 & 0.196 & 0.300\\
  &   &   & weight & \textbf{0.651} & \textbf{0.534} & 0.305 & \textbf{0.568} & 0.206 & 0.235 & 0.329\\
  & \multirow{9}{*}{\sgns} & \multirow{3}{*}{none} & prob. & 0.535 & 0.470 & \textbf{0.358} & 0.456 & \textbf{0.215} & \textbf{0.286} & 0.123\\
  &   &   & none & 0.569 & 0.515 & 0.325 & 0.493 & \textbf{0.219} & \textbf{0.285} & 0.130\\
  &   &   & weight & 0.528 & 0.456 & 0.343 & 0.450 & 0.127 & 0.159 & 0.059\\
  &   & \multirow{3}{*}{prob.} & prob. & 0.551 & 0.486 & \textbf{0.363} & 0.479 & 0.192 & 0.243 & 0.091\\
  &   &   & none & 0.576 & 0.505 & 0.320 & 0.518 & 0.182 & 0.215 & 0.087\\
  &   &   & weight & 0.531 & 0.470 & 0.322 & 0.466 & 0.116 & 0.104 & 0.052\\
  &   & \multirow{3}{*}{weight} & prob. & 0.497 & 0.453 & 0.317 & 0.444 & 0.191 & 0.267 & 0.172\\
  &   &   & none & 0.529 & 0.479 & 0.352 & 0.466 & 0.195 & 0.260 & 0.139\\
  &   &   & weight & 0.508 & 0.461 & 0.278 & 0.440 & 0.122 & 0.171 & 0.131\\
  & \glove &   & weight & 0.518 & 0.470 & 0.182 & 0.383 & 0.120 & 0.165 & \textbf{0.330}\\


  \hline

 \multirow{12}{*}{news} & \multirow{9}{*}{\svdpmi} & \multirow{3}{*}{none} & prob. & 0.776 & 0.560 & 0.417 & 0.643 & 0.467 & 0.392 & 0.654\\
  &   &   & none & 0.775 & 0.559 & 0.406 & 0.643 & 0.469 & 0.357 & \textbf{1.000}\\
  &   &   & weight & 0.776 & 0.561 & 0.417 & 0.642 & 0.473 & 0.395 & \textbf{1.000}\\
  &   & \multirow{3}{*}{prob.} & prob. & 0.784 & 0.561 & 0.431 & 0.666 & 0.492 & 0.445 & 0.654\\
  &   &   & none & 0.786 & 0.572 & 0.423 & 0.668 & 0.504 & 0.420 & 0.801\\
  &   &   & weight & \textbf{0.786} & 0.569 & 0.434 & 0.668 & 0.504 & 0.449 & 0.806\\
  &   & \multirow{3}{*}{weight} & prob. & 0.783 & 0.561 & 0.433 & 0.666 & 0.492 & 0.440 & 0.681\\
  &   &   & none & 0.785 & 0.574 & 0.424 & 0.666 & 0.503 & 0.413 & \textbf{1.000}\\
  &   &   & weight & 0.786 & 0.568 & 0.435 & 0.667 & 0.502 & 0.444 & \textbf{1.000}\\
  & \multirow{2}{*}{\sgns} &  \multirow{2}{*}{prob.} & prob. & 0.739 & 0.675 & 0.430 & 0.672 & \textbf{0.643} & 0.553 & 0.652\\
  &   &   & none & 0.738 & \textbf{0.681} & 0.408 & \textbf{0.678} & 0.635 & 0.521 & 0.657\\
  & \glove &   & weight & 0.698 & 0.576 & 0.309 & 0.536 & 0.548 & 0.444 & 0.679\\
\hline
\multirow{12}{*}{{\parbox{1cm}{\center NEWS Subs.}}} & \multirow{9}{*}{\svdpmi} & \multirow{3}{*}{none} & prob. & 0.769 & 0.556 & 0.411 & 0.619 & 0.441 & 0.370 & 0.557\\
  &   &   & none & 0.771 & 0.558 & 0.401 & 0.623 & 0.445 & 0.335 & 0.584\\
  &   &   & weight & 0.773 & 0.556 & 0.412 & 0.624 & 0.451 & 0.373 & 0.605\\
  &   & \multirow{3}{*}{prob.} & prob. & 0.776 & 0.564 & 0.423 & 0.642 & 0.463 & 0.420 & 0.571\\
  &   &   & none & \textbf{0.782} & 0.569 & 0.415 & 0.646 & 0.480 & 0.397 & 0.598\\
  &   &   & weight & \textbf{0.782} & 0.570 & \textbf{0.430} & \textbf{0.654} & 0.478 & 0.425 & 0.616\\
  &   & \multirow{3}{*}{weight} & prob. & 0.776 & 0.563 & \textbf{0.427} & 0.643 & 0.460 & 0.413 & 0.587\\
  &   &   & none & \textbf{0.781} & 0.571 & 0.417 & 0.645 & 0.476 & 0.390 & 0.617\\
  &   &   & weight & \textbf{0.781} & 0.567 & \textbf{0.430} & \textbf{0.649} & 0.476 & 0.421 & \textbf{0.635}\\
  & \multirow{2}{*}{\sgns} & \multirow{3}{*}{prob.} & prob. & 0.734 & 0.673 & 0.417 & \textbf{0.647} & \textbf{0.601} & 0.513 & 0.452\\
  &   &   & none & 0.733 & \textbf{0.680} & 0.394 & \textbf{0.651} & 0.592 & 0.483 & 0.456\\
  & \glove &   & weight & 0.687 & 0.572 & 0.301 & 0.508 & 0.505 & 0.408 & 0.461\\
  
  \hline
 
 \multirow{5}{*}{WIKI} 
& \multirow{3}{*}{\svdpmi} &  \multicolumn{2}{c|}{none} & 0.731 & 0.510 & 0.353 & 0.715 & 0.432 & 0.246 & \textbf{1.000}\\
&   &  \multicolumn{2}{c|}{prob.} & \textbf{0.747} & 0.571 & 0.392 & \textbf{0.718} & 0.482 & 0.311 & 0.714\\
&   &  \multicolumn{2}{c|}{weight} & 0.743 & 0.560 & \textbf{0.393} & \textbf{0.717} & 0.482 & 0.305 & \textbf{1.000}\\
& \multirow{1}{*}{\sgns} &  \multicolumn{2}{c|}{prob.} & 0.735 & \textbf{0.659} & 0.372 & \textbf{0.717} & \textbf{0.669} & \textbf{0.421} & 0.488\\
& \glove &  \multicolumn{2}{c|}{weight} & 0.744 & 0.651 & 0.354 & 0.667 & 0.653 & 0.397 & 0.666\\

\hline
 \multirow{5}{*}{{\parbox{1cm}{\center WIKI Subs.}}} 
& \multirow{3}{*}{\svdpmi} &  \multicolumn{2}{c|}{none} & 0.726 & 0.526 & 0.355 & 0.699 & 0.410 & 0.244 & 0.635\\
&   &  \multicolumn{2}{c|}{prob.} & \textbf{0.742} & 0.568 & \textbf{0.391} & \textbf{0.706} & 0.448 & 0.304 & 0.604\\
&   &  \multicolumn{2}{c|}{weight} & 0.740 & 0.555 & \textbf{0.389} & \textbf{0.704} & 0.451 & 0.300 & \textbf{0.651}\\
& \multirow{1}{*}{\sgns} &  \multicolumn{2}{c|}{prob.} & 0.723 & \textbf{0.657} & 0.364 & 0.686 & \textbf{0.629} & \textbf{0.407} & 0.501\\
 & \glove &  \multicolumn{2}{c|}{weight} & 0.735 & 0.642 & 0.345 & 0.655 & 0.599 & 0.382 & 0.486\\
 \hline
 
\end{tabular}
\vspace*{-5pt}
\caption{Performance of different algorithms and down-sampling strategies with models trained on corpora with and without subsampling. \textbf{Bold} values are best or not significantly different by independent t-tests (with $p < 0.05$) for the subsampled, respectively non-subsampled condition of each corpus.}\label{tab:results-short}
\end{table*} 
